Seeing and Hearing Egocentric Actions: How Much Can We Learn?

Our interaction with the world is an inherently multimodal experience. However, the understanding of human-to-object interactions has historically been addressed focusing on a single modality. In particular, a limited number of works have considered to integrate the visual and audio modalities for this purpose. In this work, we propose a multimodal approach for egocentric action recognition in a kitchen environment that relies on audio and visual information. Our model combines a sparse temporal sampling strategy with a late fusion of audio, spatial, and temporal streams. Experimental results on the EPIC-Kitchens dataset show that multimodal integration leads to better performance than unimodal approaches. In particular, we achieved a 5.18% improvement over the state of the art on verb classification.

==> subTabAction.tex <==
\multirow{7}{*}{\rotatebox{90}{\textbf{ACTION}}}%
& \textbf{Audio}%
& & VGG-11%
& \textcolor{TableGray}{33.03} & \textcolor{TableGray}{08.71} & 10.16%
& \textcolor{TableGray}{77.58} & \textcolor{TableGray}{24.67} & 26.36%
& \textcolor{TableGray}{04.02} & \textcolor{TableGray}{03.95} & 01.45%
& \textcolor{TableGray}{07.16} & \textcolor{TableGray}{05.06} & 01.84 \\\cline{2-16}
& & & TSN Flow%
& \textcolor{TableGray}{38.06} & \textcolor{TableGray}{15.46} & 25.44%
& \textcolor{TableGray}{82.11} & \textcolor{TableGray}{45.29} & 47.51%
& \textcolor{TableGray}{13.27} & \textcolor{TableGray}{14.28} & 07.45%
& \textcolor{TableGray}{12.20} & \textcolor{TableGray}{10.32} & 07.74 \\
& \textbf{Vision}%
& & TSN RGB%
& \textcolor{TableGray}{37.26} & \textcolor{TableGray}{\textbf{41.44}} & 37.23%
& \textcolor{TableGray}{83.98} & \textcolor{TableGray}{75.06} & 67.09%
& \textcolor{TableGray}{\textbf{16.52}} & \textcolor{TableGray}{45.83} & 18.34%
& \textcolor{TableGray}{\textbf{13.75}} & \textcolor{TableGray}{\textbf{35.59}} & \textbf{21.97} \\
& & & RGB+Flow%
& \textcolor{TableGray}{39.99} & \textcolor{TableGray}{40.43} & 42.51%
& \textcolor{TableGray}{85.34} & \textcolor{TableGray}{73.70} & 68.42%
& \textcolor{TableGray}{14.09} & \textcolor{TableGray}{47.06} & \textbf{21.37}%
& \textcolor{TableGray}{13.45} & \textcolor{TableGray}{32.93} & 21.86 \\ \cline{2-16}
%
& &%
& Flow+Audio%
& \textcolor{TableGray}{39.01} & \textcolor{TableGray}{15.82} & 27.28%
& \textcolor{TableGray}{82.82} & \textcolor{TableGray}{45.59} & 48.64%
& \textcolor{TableGray}{11.50} & \textcolor{TableGray}{15.40} & 07.69%
& \textcolor{TableGray}{10.63} & \textcolor{TableGray}{10.45} & 06.77 \\
& \multirow{4}{*}{\textbf{Multimodal}}%
& & RGB+Audio%
& \textcolor{TableGray}{38.98} & \textcolor{TableGray}{41.26} & 41.00%
& \textcolor{TableGray}{85.72} & \textcolor{TableGray}{75.21} & 68.51%
& \textcolor{TableGray}{13.82} & \textcolor{TableGray}{46.05} & 19.09%
& \textcolor{TableGray}{11.50} & \textcolor{TableGray}{33.92} & 19.24 \\
& & & RGB+Flow+Audio%
& \textcolor{TableGray}{\textbf{41.41}} & \textcolor{TableGray}{39.40} & 43.75%
& \textcolor{TableGray}{85.57} & \textcolor{TableGray}{72.96} & 67.92%
& \textcolor{TableGray}{11.37} & \textcolor{TableGray}{47.40} & 20.96%
& \textcolor{TableGray}{12.72} & \textcolor{TableGray}{30.84} & 19.53 \\ \cline{3-16}
%
& &\multirow{3}{*}{\rotatebox{90}{\footnotesize Weighted}}%
& Flow+Audio%
& \textcolor{TableGray}{39.37} & \textcolor{TableGray}{16.00} & 28.08%
& \textcolor{TableGray}{82.73} & \textcolor{TableGray}{46.24} & 49.64%
& \textcolor{TableGray}{11.62} & \textcolor{TableGray}{15.55} & 08.13%
& \textcolor{TableGray}{11.08} & \textcolor{TableGray}{10.48} & 07.19 \\
& & & RGB+Audio%
& \textcolor{TableGray}{39.40} & \textcolor{TableGray}{41.35} & 41.23%
& \textcolor{TableGray}{85.60} & \textcolor{TableGray}{\textbf{75.27}} & \textbf{69.11}%
& \textcolor{TableGray}{13.71} & \textcolor{TableGray}{45.60} & 19.42%
& \textcolor{TableGray}{11.76} & \textcolor{TableGray}{34.04} & 19.87 \\\vspace{5mm}
& & & RGB+Flow+Audio%
& \textcolor{TableGray}{41.35} & \textcolor{TableGray}{39.60} & \textbf{43.84}%
& \textcolor{TableGray}{\textbf{85.66}} & \textcolor{TableGray}{73.10} & 68.19%
& \textcolor{TableGray}{11.33} & \textcolor{TableGray}{\textbf{47.53}} & 21.12%
& \textcolor{TableGray}{12.65} & \textcolor{TableGray}{31.04} & 19.75 \\ \cline{2-16}

==> subTabVerbPlusNoun.tex <==
\multirow{7}{*}{\rotatebox{90}{\textbf{VERB+NOUN}}}%
& \textbf{Audio}%
& & VGG-11%
& 38.51 & 13.21 & \textcolor{TableGray}{06.69}%
& 81.13 & 35.16 & \textcolor{TableGray}{18.60}%
& 17.87 & 05.28 & \textcolor{TableGray}{00.99}%
& 14.89 & 05.93 & \textcolor{TableGray}{01.06} \\ \cline{2-16}
& & & TSN Flow%
& 50.83 & 31.19 & \textcolor{TableGray}{20.11}%
& 85.84 & 59.63 & \textcolor{TableGray}{40.55}%
& 28.81 & 24.60 & \textcolor{TableGray}{05.50}%
& 23.78 & 19.60 & \textcolor{TableGray}{05.02} \\
& \textbf{Vision}%
& & TSN RGB%
& 56.07 & 59.69 & \textcolor{TableGray}{39.01}%
& 93.01 & 86.17 & \textcolor{TableGray}{67.92}%
& 53.99 & 58.83 & \textcolor{TableGray}{21.27}%
& \textbf{42.87} & 56.88 & \textcolor{TableGray}{\textbf{22.82}} \\
& & & RGB+Flow%
& 59.77 & 60.66 & \textcolor{TableGray}{41.35}%
& 93.28 & 86.88 & \textcolor{TableGray}{65.43}%
& 59.03 & 60.87 & \textcolor{TableGray}{21.54}%
& 39.51 & \textbf{57.00} & \textcolor{TableGray}{22.31} \\ \cline{2-16}
& & & RGB+Flow%
& 59.75 & 59.80 & \textcolor{TableGray}{40.76}%
& 93.10 & 85.75 & \textcolor{TableGray}{68.19}%
& 58.34 & 64.34 & \textcolor{TableGray}{20.97}%
& 36.28 & 53.77 & \textcolor{TableGray}{20.19} \\ \cline{2-16}
%
& &%
& Flow+Audio%
& 54.09 & 30.84 & \textcolor{TableGray}{20.44}%
& 87.00 & 59.48 & \textcolor{TableGray}{42.42}%
& 39.53 & 29.22 & \textcolor{TableGray}{05.82}%
& 24.44 & 17.62 & \textcolor{TableGray}{04.49} \\
& \multirow{4}{*}{\textbf{Multimodal}}%
& & RGB+Audio%
& 59.48 & 58.77 & \textcolor{TableGray}{39.78}%
& 93.31 & 85.93 & \textcolor{TableGray}{68.07}%
& 62.25 & 63.55 & \textcolor{TableGray}{21.02}%
& 37.28 & 52.86 & \textcolor{TableGray}{19.87} \\
& & & RGB+Flow+Audio%
& 62.03 & 58.41 & \textcolor{TableGray}{40.73}%
& 92.83 & 84.77 & \textcolor{TableGray}{66.71}%
& \textbf{63.99} & \textbf{67.64} & \textcolor{TableGray}{20.30}%
& 35.48 & 49.75 & \textcolor{TableGray}{18.07} \\ \cline{3-16}
%
& &\multirow{3}{*}{\rotatebox{90}{\footnotesize Weighted}}%
& Flow+Audio%
& 55.09 & 32.35 & \textcolor{TableGray}{21.77}%
& 87.06 & 60.25 & \textcolor{TableGray}{40.37}%
& 42.74 & 28.44 & \textcolor{TableGray}{06.23}%
& 25.01 & 20.10 & \textcolor{TableGray}{05.29} \\
& & & RGB+Audio%
& 60.25 & 60.19 & \textcolor{TableGray}{41.59}%
& \textbf{93.66} & 86.49 & \textcolor{TableGray}{66.26}%
& 63.27 & 60.30 & \textcolor{TableGray}{\textbf{21.91}}%
& 40.54 & \textbf{57.00} & \textcolor{TableGray}{22.28} \\
& & & RGB+Flow+Audio%
& \textbf{62.20} & \textbf{60.99} & \textcolor{TableGray}{\textbf{42.89}}%
& 92.71 & \textbf{86.91} & \textcolor{TableGray}{\textbf{68.42}}%
& 63.34 & 62.25 & \textcolor{TableGray}{21.03}%
& 35.63 & 56.65 & \textcolor{TableGray}{21.10} \\

==> tabActionRecognition.tex <==
\begin{table*}[!t]
% \vspace{-1mm}
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccl|ccc|ccc|ccc|ccc}
& & & & \multicolumn{3}{c|}{\textbf{Top-1 Accuracy}} & \multicolumn{3}{c|}{\textbf{Top-5 Accuracy}} & \multicolumn{3}{c|}{\textbf{Avg Class Precision}} &\multicolumn{3}{c}{\textbf{Avg Class Recall}} \\\cline{5-16}
& & & & VERB      & NOUN      & ACTION     & VERB      & NOUN      & ACTION     & VERB   & NOUN  & ACTION & VERB   & NOUN  & ACTION \\ \cline{4-16}
& & & Chance/Random & 12.91 & 02.44 & 00.73 & 55.16 & 11.97 & 03.61 & 03.84 & 01.41 & 00.14 & 03.84 & 01.41 & 00.15 \\ \vspace{5mm}
& & & Largest class & 21.06 & 05.33 & 02.81 & 73.73 & 23.64 & 10.10 & 00.81 & 0.08 & 00.00 & 03.85 & 01.41 & 00.16 \\ \cline{2-16}
%
%
\input{subTabAction.tex}
%
%
\input{subTabVerbPlusNoun.tex}
\end{tabular}
}
\caption{Classification performance for the equally stratified \textit{action} data split. The \textit{action} part show the results of training one classifier on the action labels, whereas the \textit{verb+noun} part show the results of independently training two classifiers over the verb and noun labels. The scores in \textcolor{TableGray}{\textbf{gray}} color were calculated based on the respective \textit{action} or \textit{verb+noun} classifiers.}
\label{tab:actionRecognition}
\end{center}
\vspace{-5mm}
\end{table*}

==> tabVerbNounRecognition.tex <==
\begin{table*}[!t]
% \vspace{-1mm}
\begin{center}
\resizebox{1.6\columnwidth}{!}{%
\begin{tabular}{ccl|cc|cc|cc|cc}
& & & \multicolumn{2}{c|}{\textbf{Top-1 Accuracy}} & \multicolumn{2}{c|}{\textbf{Top-5 Accuracy}} & \multicolumn{2}{c|}{\textbf{Avg Class Precision}} &\multicolumn{2}{c}{\textbf{Avg Class Recall}} \\ \cline{4-11}
& &                                   & VERB & NOUN & VERB & NOUN  & VERB & NOUN  & VERB & NOUN  \\ \cline{2-11}
& & Chance/Random & 13.12 & 02.46 & 55.99 & 12.04 & 03.84 & 01.41 & 03.84 & 1.41 \\
& & Largest class & 21.53 & 05.39 & 75.26 & 24.01 & 00.83 & 00.08 & 03.85 & 1.41 \\ \cline{1-11}
\textbf{Audio}& & Traditional Dilated & 37.33 & 16.98 & 81.77 & 40.72 & 17.65 & 11.44 & 12.09 & 09.45 \\
              & & VGG-11              & 39.39 & 13.41 & 81.99 & 35.60 & 16.20 & 03.85 & 14.19 & 05.48 \\ \cline{1-11}
              & & TSN Flow            & 50.86 & 33.24 & 86.65 & 59.82 & 26.77 & 31.03 & 23.73 & 21.57 \\
\textbf{Vision}& & TSN RGB            & 54.65 & 60.70 & 93.55 & 85.89 & 56.37 & 60.55 & \textbf{42.65} & \textbf{57.10} \\
% & Weighted RGB + Flow& 60.01 & 61.49 & 93.49 & 85.92 & 53.97 & 61.87 & 35.06 & 56.64 \\ \cline{1-10}
               & & RGB + Flow            & 59.82 & 60.28 & \textbf{93.58} & 85.65 & 54.32 & 65.15 & 35.82 & 53.17 \\ \cline{1-11}
\multirow{6}{*}{\textbf{Multimodal}}%
& & Flow+Audio     & 53.95 & 34.15 & 87.47 & 61.79 & 33.64 & 34.60 & 23.09 & 20.30 \\
& & RGB+Audio      & 59.64 & 61.79 & 93.31 & 85.65 & \textbf{59.12} & 66.02 & 37.21 & 55.42 \\
& & RGB+Flow+Audio & 61.94 & 59.79 & 92.79 & 85.04 & 57.50 & \textbf{67.96} & 34.00 & 50.43 \\ \cline{2-11}
% 
&\multirow{3}{*}{\rotatebox{90}{\footnotesize Weighted}} &%
    Flow+Audio     & 55.01          & 35.18 & 87.68          & 62.28 & 33.99 & 36.10 & 24.36 & 21.53 \\
& & RGB+Audio      & 59.92          & 62.03 & \textbf{93.58} & 85.98 & 58.62 & 65.33 & 38.77 & 55.99 \\
& & RGB+Flow+Audio & \textbf{62.43} & \textbf{62.13} & 92.92 & \textbf{86.10} & 59.10 & 63.52 & 35.00 & 56.36 \\
\end{tabular}
}
\caption{Classification performance for the equally stratified \textit{verb} and \textit{noun} data splits.}
\label{tab:verbNounRecognition}
\end{center}
\vspace{-5mm}
\end{table*}

==> tabVideoSegmentTimeDurationStats.tex <==
\helvetica%
\begin{center}
Video segments time duration stats (secs)\\
\begin{tabular}{r l}
\hline
\textbf{Min}: &\hspace{-2.5mm} 0.5\\
\textbf{Mean}: &\hspace{-2.5mm} 3.38\\
\textbf{Median}: &\hspace{-2.5mm} 1.78\\
\textbf{Std. Dev.}: &\hspace{-2.5mm} 5.04\\
\textbf{Mode}: &\hspace{-2.5mm} 1.0\\
\textbf{Max}: &\hspace{-2.5mm} 145.16\\
\end{tabular}
\end{center}%
